First Multi-Dimensional Evaluation of Flowchart Comprehension for Multimodal Large Language Models

With the development of Multimodal Large Language Models (MLLMs) technology, its general capabilities are increasingly powerful. To evaluate the various abilities of MLLMs, numerous evaluation systems have emerged. But now there is still a lack of a comprehensive method to evaluate MLLMs in the tasks related to flowcharts, which are very important in daily life and work. We propose the first comprehensive method, FlowCE, to assess MLLMs across various dimensions for tasks related to flowcharts. It encompasses evaluating MLLMs' abilities in Reasoning, Localization Recognition, Information Extraction, Logical Verification, and Summarization on flowcharts. However, we find that even the GPT4o model achieves only a score of 56.63. Among open-source models, Phi-3-Vision obtained the highest score of 49.97. We hope that FlowCE can contribute to future research on MLLMs for tasks based on flowcharts. \url{https://github.com/360AILABNLP/FlowCE}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
% \begin{abstract}
% The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
% Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
% The abstract is to be in 10-point, single-spaced type.
% Leave two blank lines after the Abstract, then begin the main text.
% Look at previous \confName abstracts to get a feel for style and length.
% \end{abstract}

\begin{abstract}
With the development of Multimodal Large Language Models (MLLMs) technology, its general capabilities are increasingly powerful. To evaluate the various abilities of MLLMs, numerous evaluation systems have emerged. But now there is still a lack of a comprehensive method to evaluate MLLMs in the tasks related to flowcharts, which are very important in daily life and work. We propose the first comprehensive method, FlowCE, to assess MLLMs across various dimensions for tasks related to flowcharts. It encompasses evaluating MLLMs' abilities in Reasoning, Localization Recognition, Information Extraction, Logical Verification, and Summarization on flowcharts. However, we find that even the GPT4o model achieves only a score of 56.63. Among open-source models, Phi-3-Vision obtained the highest score of 49.97. We hope that FlowCE can contribute to future research on MLLMs for tasks based on flowcharts. \url{https://github.com/360AILABNLP/FlowCE}
\end{abstract}

==> sec/1_intro.tex <==
% \section{Introduction}
% \label{sec:intro}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}
\section{Introduction}
In the modern work environment, flowcharts have become a widely used graphical tool across various industries and fields. Flowcharts provide an intuitive and efficient way to describe and analyze workflows. By representing processes graphically, complex workflows can be simplified into easily understandable steps, thereby facilitating a range of tasks. Currently, leveraging Multimodal Large Language Models (MLLMs) for the understanding and analysis of flowcharts has become a research focus. Represented by models like GPT-4v \cite{gpt4}, these large models can comprehend user-input images and perform corresponding question-and-answer tasks. Meanwhile, there have been numerous open-source efforts for MLLMs, such as LLAVA-1.6v \cite{lava1.6}, QWEN-VL \cite{qwenvl}, MiniCPM \cite{minicpm}, phi-3-vision \cite{phi3}, and CogVLM2 \cite{cogvlm}. To evaluate the cross-modal understanding capabilities of existing MLLMs between images and text, various benchmarks have emerged, including MMBench \cite{mmbench}, MME \cite{mme}, TextVQA \cite{singh2019towards}, MM-Vet \cite{mm-vet}, DocVQA \cite{docvqa}, ChartQA \cite{chartqa}, InfographicQA \cite{infographicvqa}, FlowChartQA \cite{flowchartqa} and so on. Additionally, these evaluation systems measure the capabilities of MLLMs from different perspectives, including the understanding of general images, document-type images, chart-type images, and more.

\begin{figure}[t]
\hspace*{-7.0mm}
\centering
\includegraphics[width=2.8in]{latex/img/radar.pdf}
    \caption{Evaluation results of multimodal large language models on five dimensions of tasks in FlowCE. GPT-4o achieves the highest overall score of 56.63.}
\label{fig:1}
\vspace{-6mm}
\end{figure}

\begin{table*}[!ht]
    \centering
    \small
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{ccccccccccc}
    \hline
        Benchmark & Capability & Real-world Data & Handcrafted Questions & Answer Type & Size & \# models  \\ \hline
        LVLM-eHub & General Multi-Modality & \ding{51} &  \ding{115} & MC/OE & 332k &  8 \\ 
        MME & General Multi-Modality & \ding{51} & \ding{51} & MC & 2,194 &  10  \\ 
        MMBench & General Multi-Modality & \ding{51} &  \ding{115} & MC & 2,974 &  14  \\ 
        TextVQA & Text Recognition and  Contextual Reasoning & \ding{51} & \ding{51} & OE & 45.3k &  6 \\ 
        InfographicVQA & Integrated Document Visual and Textual Reasoning & \ding{51} & \ding{51} & OE & 30k &  1  \\ 
        ChartQA & Chart Understanding and Analysis & \ding{51} & \ding{51} & OE & 9.6k &    4 \\ 
        MathVista & Mathematical Reasoning & \ding{51} & \ding{51} & MC & 6141 &  11  \\ 
        EgoThink & First-Person Thinking & \ding{51} & \ding{51} & OE & 700 &  21  \\ 
        FlowchartQA & Geometirc and Topological Information of Flowcharts & \ding{55} & \ding{55} & MC & 6M &   1 \\
        FlowVQA & Understanding of Flowcharts & \ding{55} & \ding{55} & MC/OE & 22k & 6 \\
        FlowCE(ours) & Comprehensive Understanding of Flowcharts   & \ding{51} & \ding{51} & MC/OE & 505 & 19 \\ \hline
    \end{tabular}
    }
    \caption{Comparison of recent comprehensive evaluation benchmarks of MLLMs and our proposed benchmark FlowCE. MC/OE indicate multi-choice and open-ended question-answering respectively. "\ding{115}" indicates that there are both handcrafted questions and questions generated using templates.  }
    \vspace{-2mm}
    \label{table:detailed-dataset-info}
\end{table*}

However, to the best of our knowledge, none of these existing evaluation benchmarks comprehensively assess MLLMs' understanding of flowcharts from multiple perspectives in real-world scenarios. This hinders the development of methods for utilizing MLLMs to understand and analyze flowcharts in open environments. Thus, inspired by previous works such as FigureQA \cite{figureqa}, PlotQA \cite{plotqa}, ChartQA \cite{chartqa} and FlowchartQA \cite{flowchartqa}, and motivated by the successful development of MLLMs. We propose a novel benchmark, FlowCE, for the first time: comprehensively assessing the understanding capabilities of multimodal large language models on flowcharts in real-world scenarios. FlowCE evaluates the understanding capabilities of existing MLLMs on flowcharts from multiple dimensions, including Reasoning, Information Extraction, Localization Recognition, Summarization, and Logical Verification. We have carefully designed diverse question-answer pairs for various dimensional tasks in open environments. Additionally, the flowchart images in FlowCE are sourced from a variety of real-world scenarios and styles. We have carefully designed diverse question-answer pairs for various dimensional tasks in open environments. Additionally, the flowchart images in FlowCE are sourced from a variety of real-world scenarios and styles. 

We conducted evaluations on all mainstream MLLMs, both open-source and proprietary, using FlowCE. The evaluation results for some parts on FlowCE are shown in Figure \ref{fig:1}. The results indicate that even the highly performant GPT4o achieves only a score of 56.63, with the best performance among open-source models being achieved by Phi-3-Vision \cite{phi3}, scoring 49.97. Our main contributions are as follows:

\begin{itemize}
\vspace{-1mm}
    {
    \item 
    We introduce FlowCE to comprehensively evaluate the understanding capabilities of MLLMs on flowcharts. It encompasses evaluation tasks and methodologies across dimensions such as reasoning, information extraction, localization recognition, summarization, and logical verification.
    \item 
    We extensively evaluate mainstream open-source and proprietary models using FlowCE. Through detailed analysis of these MLLMs' performance across different dimensional tasks, we uncovered their strengths and limitations in understanding flowcharts. Additionally, we proposed some improvement suggestions for existing models to facilitate future research and development. 
    \item 
    We are open-sourcing our resources to foster future advancements in this field.
    }
\end{itemize}


==> sec/2_related.tex <==
% \section{Formatting your paper}
% \label{sec:formatting}

% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

\section{Related Work}

\subsection{Multimodal Large Language Models}

Inspired by the remarkable success of LLMs such as internVL \cite{chen2024internvl}, llama3 \cite{touvron2023llama}, Yi-chat \cite{young2024yi}, Qwen \cite{qwen}, and Vicuna \cite{zheng2024judging_vicuna}, recent MLLMs have incorporated these advanced LLMs as their primary backbone. Examples include the LLAVA-V1.6 \cite{liu2024llava} series, ShareGPT4 \cite{chen2023sharegpt4v} series, Qwen \cite{qwenvl} series, Cogvlm \cite{cogvlm} series and so on. Initially, MLLMs leverage vast datasets consisting of image-text pairs \cite{alayrac2022flamingo,zhu2024multimodal} or an arbitrarily combination of visual and textual data for pre-training \cite{li2023mimic, liu2024improved}. Moreover, the availability of extensive image-text instruction datasets facilitate recent studies \cite{dai2024instructblip, li2023mimic,liu2024visual,ye2023mplug,chen2023sharegpt4v} to implement instruction tuning. This fine-tuning process enhances the ability of MLLMs to produce high-quality responses. This two-phase training strategy  \cite{li2022overcoming, yang2022multimodal} enables recent MLLMs to achieve outstanding performance in downstream vision-language tasks \cite{antol2015vqa, hudson2019gqa, lin2014microsoft, plummer2015flickr30k}.

\subsection{Benchmarks for MLLMs}

\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=0.8\textwidth]{latex/img/flowce-progress-V2.pdf} 
    \caption{The process of creating and evaluating FlowCE. }
    \label{fig:FlowCE-process-evaluate}
    \vspace{-3mm}
\end{figure*}


To evaluate the capabilities of Vision-Language Models (MLLMs), various downstream language tasks are employed. General benchmarks, such as MMBench \cite{mmbench}, MME \cite{mme}, and LVLM-ehub \cite{Lvlmehub}, provide a comprehensive assessment of model performance. Domain-specific benchmarks, such as TextVQA \cite{singh2019towards} and DocVQA \cite{docvqa}, evaluate the fine-grained transcription capabilities of MLLMs on low-resolution images. MathVista \cite{lu2024mathvista} examines the ability of MLLMs to integrate visual and mathematical logic. ChartQA \cite{chartqa} aims to evaluate direct chart understanding and analysis, while InfographicQA \cite{infographicvqa} addresses logical questions about data visualizations and charts. EgoThink \cite{cheng2024egothink} elaborate on the capabilities of MLLMs to think from a first-person perspective. General benchmarks offer a broad and consistent evaluation framework \cite{Lvlmehub, mme, mmbench}, whereas domain-specific benchmarks enable detailed assessment of model capabilities and promote advancements in specific research areas.



In Table \ref{table:detailed-dataset-info}, we compare FlowCE with various existing benchmarks. FlowCE comprehensively assesses for the first time the ability of MLLMs to understand flowcharts. Specifically, compared to FlowchartQA \cite{flowchartqa}, we not only introduce tasks across more dimensions but also create real-world flowchart data and open-scenario question-answer pairs. Compared to FlowVQA \cite{singh-etal-2024-flowvqa} , we have collected real-world flowcharts rather than relying solely on a single style of flowchart rendered by Mermaid. In contrast to GPT-generated question-answer pairs, our dataset employs human-generated question-answer pairs, offering greater diversity and textual richness.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{latex/img/flowce-example.pdf} 
    \caption{Data samples of FlowCE, which covers 5 evaluation dimensions. Each evaluation dimension contains human-annotated question-answer pairs.}
    \label{fig:FlowCE-example}
    \vspace{-3mm}
\end{figure*}



==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_flowce.tex <==
\section{FlowCE}
In this section, we elaborate first on the evaluation tasks across various dimensions in FlowCE. Then, we introduce the process of manually constructing diverse open-scenario question-answer pairs. Finally, we present the evaluation methodologies for tasks across different dimensions. The process of creating and evaluating FlowCE is illustrated in Figure \ref{fig:FlowCE-process-evaluate}. Using \textit{flowchart} as the keyword, an initial screening of 6,562 links was performed via the Baidu and Google search engines. After removing duplicates and irrelevant results, 500 images were selected. These images were randomly divided into five categories of questions: Logical Verification (LV), Information Extraction (IE), Localization Recognition (LR), Reasoning (RS), and Summarization (SM), with 100 images in each category. A human annotator manually generated questions and answers for each major category, which were then reviewed by annotators from other categories. The final annotations were unanimously agreed upon by five annotators. The RS, LR, and SM tasks were evaluated using LLM-based scoring, while LV and IE tasks were assessed using rule-based scoring. We also conducted a validity assessment of the LLM-based scoring, achieving an average consistency of 0.9451.

\subsection{Tasks across different dimensions}
As shown in Figure \ref{fig:FlowCE-example}, we establish tasks across five dimensions in real flowchart scenarios, including reasoning, information extraction, localization recognition, summarization, and logical verification, for quantitative evaluation.
\\
\textbf{Logical Verification} \quad  Upon receiving a process diagram, users provide the logical relationships between different nodes or boxes in the diagram, and MLLMs are tasked with evaluating these relationships. Figure \ref{fig:FlowCE-example}(a) shows an example of Logical Verification. This process entails a comprehensive analysis of the structure and content of the process diagram to ensure the accuracy and coherence of the logical relationships. MLLMs assess whether the provided process logic aligns with the actual scenario by considering the interactions among individual nodes and their roles throughout the entire process.
\\
\textbf{Information Extraction} \quad The task entails MLLMs receiving flowchart images and extracting corresponding textual information based on user queries. We have categorized the questions into two main types based on the content of the flowchart: the first type involves prompting MLLMs to extract all textual information from the flowchart, while the second type entails extracting specific textual information based on the characteristics of the flowchart. An example of Information Extraction is shown in Figure \ref{fig:FlowCE-example}(b).
\\
\textbf{Localization Recognition} \quad  Users will inquire about the positional relationships between different nodes or boxes in the flowchart, an example of Localization Recognition is illustrated in Figure \ref{fig:FlowCE-example}(c), thereby assessing whether MLLMs have an accurate understanding of the positional relationships of nodes and boxes in the flowchart.
\\
\textbf{Reasoning} \quad For an example of Reasoning, as shown in Figure \ref{fig:FlowCE-example}(d), the task refers to MLLMs making decisions in response to user inquiries based on the content of the flowchart images after being provided with them. Here, we formulate more natural questions based on the content of the flowchart, which require judgment and reasoning considering aspects such as conditional relationships within the flowchart to answer, rather than relying solely on the direction of the arrows in the flowchart.
\\
\textbf{Summarization} \quad  MLLMs provide a summarized abstraction of the content depicted in process diagrams, elucidating the conveyed information. They accomplish this task by analyzing the logical relationships among various nodes within the diagram, identifying key steps and critical information, and integrating them into a concise yet comprehensive summary. Through understanding and encapsulating the process diagram, MLLMs generate the primary flow of the process and key decision points, thereby assisting users in better comprehending the process or system represented by the diagram, as shown in Figure \ref{fig:FlowCE-example}(e).

\subsection{Data construction}
In this section, we introduce the data of FlowCE and elaborate on the detailed process of constructing FlowCE.
\\
\textbf{FlowCE-data} \quad FlowCE is built upon 500 real-world flowcharts, ensuring an ample diversity in each chart. In Figure \ref{distribution-a}, we present a detailed breakdown of the category distribution within the flowchart, encompassing categories from daily life, various specialized filed flowcharts, coding flowcharts, mathematical flowcharts, and others. As shown in Figure \ref{resolution-b}, the most common HD and Full HD images in daily life account for the majority of FlowCE, while other types of resolution images also have a share, indicating the diversity of FlowCE resolutions. As shown in Figure \ref{cumulative-frequency-c}, under the same data scale, FlowCE exhibits a longer growth trajectory compared to FlowVQA, featuring richer and more diverse vocabulary. Numerically, FlowVQA has 5,847 tokens, while FlowCE contains 7,106. Additional details about the dataset can be found in \ref{appendix:diverse analyses of dataset}.
\\
\textbf{Human-annotated} \quad To ensure an open-ended question-and-answer format, we manually constructed question-answer pairs for each flowchart. We assigned different dimensions of tasks to the same individual to annotate a particular type of question, ensuring consistency in the tasks. Additionally, to allow for greater diversity in open-ended question-and-answer scenarios, we leveraged powerful GPT-like models for auxiliary construction, aiding humans in exploring more imaginative possibilities. Please refer to the Appendix \ref{sec:appendix} for specific details.


\begin{figure*}
    \centering
    \begin{minipage}{0.26\textwidth}
        \centering
        \includegraphics[width=\textwidth]{latex/img/flowchart_distribution_pie.pdf}
        \subcaption{Flowchart Type Distribution Across Varied Categories.}
        \label{distribution-a}
    \end{minipage}
    \hspace{1em}
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{latex/img/static-resolution.pdf}
        \subcaption{Resolution Distribution in Flowchart Representation.}
        \label{resolution-b}
    \end{minipage}
    \hspace{1em}
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{latex/img/static-cumulative-frequency.pdf}
        \subcaption{Cumulative Word Frequency Distribution of FlowCE and FlowVQA.  FlowCE exhibits a longer growth trajectory compared to FlowVQA, featuring richer and more diverse vocabulary.}
        \label{cumulative-frequency-c}
    \end{minipage}
    \vspace{-0.5em}
    \caption{The statistics information of FlowCE.}
    \label{statistics infomation of FlowCE}
    \vspace{-3mm}
\end{figure*}
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{latex/img/flowchart_distribution_pie.pdf}
%     \caption{Distribution of Different Types of Flowcharts}
%     \label{distribution}
% \end{figure}


\subsection{Evaluation method}
In this section, the evaluation of various tasks quantification methods will be introduced.
\\
\textbf{Automatic evaluation} \quad For tasks involving open-ended question answering, such as reasoning, localization recognition, and summarization, we employ GPT4 to assess the semantic similarity between standard answers and the responses generated by MLLMs. For detailed methodology of the evaluation utilizing GPT4, please refer to the Appendix \ref{appendix:Large Language Model Judge}.
\\
\textbf{Accuracy calculation} \quad Firstly, for the logical verification task, we match the output of MLLMs, either \textit{"Yes"} or \textit{"No,"} with the standard answers to calculate the accuracy after all questions have been answered, thereby quantifying the score of MLLMs on this task. Next, for the information extraction task, we propose a method based on effective factor to fairly compare the content generation effectiveness of different MLLMs. Then, for the information extraction task, we propose a method based on the effective factor to fairly compare the performance of different MLLMs in generating content. Suppose the label set is given by $\text{label} = [\text{text}_1, \text{text}_2, \ldots, \text{text}_n]$, where $\text{text}_n$ represents the $n$-th text. The output answers are given by $\text{prediction} = [\text{pre}_1, \text{pre}_2, \ldots, \text{pre}_m]$, where $\text{pre}_m$ is the $m$-th predicted text. If there is a predicted text in $\text{prediction}$ that does not exist in $\text{label}$, and there are $t$ such texts ($t \geq 1$), then the effective factor $\delta$ changes according to the following formula:
\[
\delta = \delta^t,
\]
At this point, if there is a predicted text in $\text{prediction}$ that exists in $\text{label}$, then the initial score $s$ changes as follows:
\[
s = s \cdot \delta,
\]

If $t = 0$, then for each predicted text in $\text{prediction}$ that exists in $\text{label}$, the score remains the initial score $s$. Suppose there are $i$ predicted texts that exist in $\text{label}$, the total score is $s \cdot i$. The product of the number of texts in $\text{label}$ and the initial score is denoted as $a$. The quantitative score for evaluating MLLMs on this task is given by:
\[
\text{Score} = \frac{s \cdot i}{a} (\%).
\]

\renewcommand{\arraystretch}{1.2} 
\begin{table*}[!ht]
    \centering
   % \small
    \large
     \adjustbox{max width=\textwidth}{
     
    \begin{tabular}{ccccccc}
    \hline
        \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Image Encoder}} & \multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{Alignment Module}} & \multirow{2}{*}{\textbf{ToP}} & \multicolumn{2}{c}{\textbf{Dataset Size}} \\ \cline{6-7}
    & & & & & Pretraining & Finetuning \\ 
        % Models & Image Encoder & LLM & Alignment Module & ToP & pretraining dataset & finetuning dataset \\ 
        \hline
        \rowcolor{gray!5}
        \multicolumn{7}{c}{\textbf{API-based (Proprietary) Models}}  \\
        \hline

         GPT4o \cite{gpt4} & \multicolumn{6}{c}{\multirow{3}{*}{/}} \\ 
         GPT4V \cite{gpt4} & \multicolumn{6}{c}{} \\ 
         Qwen-VL-MAX  \cite{qwenvl} & \multicolumn{6}{c}{} \\ 

        \hline
        \rowcolor{gray!5}
        \multicolumn{7}{c}{\textbf{3.4B$\sim$7B Models}}  \\
        \hline
        MiniCPM-V2 \cite{minicpm} & SigLip-400M & MiniCPM-2.4B & RLHF-V \cite{yu2024rlhf} & 3.43B & / & / \\ 
        Phi-3-Vision \cite{phi3} & CLIP-ViT-L-336px & phi-3-mini-128K-instruct & SFT+DPO & 4.2B & 0.5T & 15B \\ 
        LLAVA-V1.5-7B \cite{liu2024improved} & CLIP-ViT-L-336px & Llama2-7B & MLP & 7.1B & 558K & 665K \\ 
        ShareGPT4V-7B \cite{chen2023sharegpt4v} & CLIP-ViT-L-336px & Vicuna-7B & MLP & 6.7B & 1.2M & 665K \\ 
        LLAVA-V1.6-7B \cite{liu2024llava} & CLIP-ViT-L-336px & Vicuna-7B & Linear & 7.06B & 558K & 760K \\ 
        \hline
        \rowcolor{gray!5}
        \multicolumn{7}{c}{\textbf{8B$\sim$13B Models}}  \\
        \hline
        LLAVA-Llama3-8B \cite{contributors2023xtuner}  & CLIP-ViT-L-336px & Llama3-8B-Instruct & MLP & 8.03B & 558K & 665K \\ 
        MiniCPM-Llama3-V2.5 \cite{minicpm} & SigLip-400M & Llama3-8B-Instruct & RLAIF-V \cite{yu2024rlaif}& 8.54B & / & / \\ 
        Qwen-Chat-VL \cite{qwenvl} & Open-CLIP-bigG & Qwen-7B & Cross-Attention & 9.6B & 1.4T & 76.8M \\ 
        LLAVA-V1.5-13B \cite{liu2024improved} & CLIP-ViT-L-336px & Llama2-13B & MLP & 13.3B & 558K & 665K \\ 
        ShareGPT4V-13B \cite{chen2023sharegpt4v} & CLIP-ViT-L-336px & Vicuna-13B & MLP & 12.58B & 1.2M & 665K \\ 
        LLAVA-V1.6-13B \cite{liu2024llava} & CLIP-ViT-L-336px & Vicuna-13B & Linear & 13.3B & 558K & 760K \\ 
        \hline
        \rowcolor{gray!5}
        \multicolumn{7}{c}{\textbf{13B$\sim$ Models}}  \\
        \hline
        Cogvlm-Chat \cite{cogvlm} & EVA2-CLIP-E & CogVLM-17B & Visual Expert & 17.6B & 1.5B & / \\ 
        Cogvlm2-Llama3-Chat-19B \cite{cogvlm} & EVA2-CLIP-E & Meta-Llama-3-8B-Instruct & Visual Expert & 19.5B & / & / \\ 
        LLAVA-Internlm2-Chat-20B \cite{contributors2023xtuner} & CLIP-ViT-L-336px & InternLM2-Chat-20B & deepspeed finetuning & 20B & 595K & 150K \\ 
        LLAVA-Next-Yi-34B \cite{liu2024llava} & CLIP-ViT-L-336px & Nous-Hermes-2-Yi-34B & Linear & 34.8B & 558K & 760K \\ 
        Yi-VL-34B \cite{young2024yi} & CLIP-ViT-L-336px & Yi-34B-Chat & MLP & 34B & 3.1T & 1.25M \\ \hline
    \end{tabular}
        }
        \caption{Statistics of compared API-based and open-source MLLMs, where ToP indicates Total Parameters and '/' indicates no detailed information for now.}
        \label{table:model-training-dataset}
        \vspace{-3mm}
\end{table*}


==> sec/4_exper.tex <==
\section{Experiments}

\begin{table*}[h]
\centering
% \resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3pt}
\begin{adjustbox}{max width=\textwidth}
\small
\begin{tabularx}
{\textwidth}
{>{\centering\arraybackslash}m{4.5cm}>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}m{1.25cm}}
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{5}{c}{\textbf{FlowCE}} & \multirow{2}{*}{\textbf{Average}} \\
\cline{2-6}
& \textbf{LV} & \textbf{IE} & \textbf{RS} & \textbf{LR} & \textbf{SM} & \\
\hline
\rowcolor{gray!5}
\multicolumn{7}{c}{\textbf{API-based Models}}  \\
\hline
GPT4o & \textbf{83.81} & \underline{17.04} & \underline{57.60} & 44.80 & \underline{79.90} & \color{red}{56.63} \\
GPT4V & \underline{77.14} & 12.94 & \textbf{59.40} & \underline{45.80} & \textbf{82.40} & 55.54 \\
Qwen-VL-MAX & 72.38 & \textbf{20.32} & 56.60 & \textbf{48.20} & 70.25 & 53.55 \\

\hline
\rowcolor{gray!5}
\multicolumn{7}{c}{\textbf{3.4B$\sim$7B Models}}  \\
\hline
MiniCPM-V2 & 51.43 & 7.00 & 30.00 & \underline{22.00} & \underline{50.20} & 32.13 \\
Phi-3-Vision  & \textbf{60.95} & \textbf{35.30} & \textbf{45.00} & \textbf{37.80} & \textbf{70.80} & \color{blue}{49.97} \\

LLAVA-V1.5-7B & \underline{53.33} & 4.90 & 14.40 & 18.20 & 35.60 & 25.29 \\
ShareGPT4V-7B & 50.48 & 3.72 & 12.20 & 16.80 & 33.60 & 23.36 \\
LLAVA-V1.6-7B  & 52.38 & \underline{7.20} & \underline{31.20} & 21.40 & 45.90 & 31.62 \\
\hline
\rowcolor{gray!5}
\multicolumn{7}{c}{\textbf{8B$\sim$13B Models}}  \\
\hline
LLAVA-Llama3-8B & 55.24 & 8.04 & 21.20 & 20.80 & 33.20 & 27.70 \\
MiniCPM-Llama3-V2.5 & \underline{58.10} & \textbf{12.25} & \textbf{45.20} & \textbf{42.80 }& 17.20 & 35.11 \\
Qwen-Chat-VL & 50.48 & 3.73 & \underline{38.80} & 23.00 & \underline{41.60} & 31.52 \\
LLAVA-V1.5-13B & 53.33 & 5.36 & 22.60 & 22.20 & 40.50 & 28.80 \\
ShareGPT4V-13B & 53.33 & 4.46 & 22.20 & 16.60 & 41.50 & 27.62 \\
LLAVA-V1.6-13B  & \textbf{62.86} & \underline{9.47} & 37.40 & \underline{27.80} & \textbf{50.70} & 37.65 \\
\hline
\rowcolor{gray!5}
\multicolumn{7}{c}{\textbf{13B$\sim$Models}}  \\
\hline
Cogvlm-Chat & 50.48 & 0.34 & 34.80 & 29.60 & 53.20 & 33.68 \\
Cogvlm2-Llama3-Chat-19B & 57.14 & 4.70 & \underline{44.60} & \textbf{37.20} & \textbf{74.30} & 43.59 \\
LLAVA-Internlm2-Chat-20B & \underline{59.05} & \underline{5.69} & 15.40 & 19.00 & 41.90 & 28.21 \\
LLAVA-Next-Yi-34B & \textbf{60.95} & \textbf{12.21} & \textbf{51.20} & \underline{34.20} & \underline{63.10} & 44.33 \\
Yi-VL-34B & \textbf{60.95} & 2.14 & 18.40 & 18.80 & 30.90 & 26.24 \\
\hline
\end{tabularx}
\end{adjustbox}
\caption{Detailed evaluation results on FlowCE across different models, where "LV" stands for Logical Verification, "IE" for Information Extraction, "RS" for Reasoning, "LR" for Localization Recognition, and "SM" for Summarization. \textbf{Bold font} indicates the best performance in the same category, while \underline{underlined font} indicates the second-best performance in the same category. \color{red}{Red} \color{black}{ indicates the  highest average score among all API-based models.} \color{blue}{Blue} \color{black}{indicates the highest average score among all open-source models.}
}
\label{tab:performance}

\end{table*}

\begin{figure*}[htb]
    \centering
    \includegraphics[width=1.0\textwidth]{latex/img/model-prediction-example-enhanced.pdf} 
    \caption{Some results from vary MLLMs. \underline{The words underlined} indicate additional prompts. (a) showcases results on Information Extraction, (b) presents results on Localization Recognition, (c) showcases results on Logical Verification, (d) showcase results on Summarization, (e) displays results on Reasoning. } 
    \label{model prediction example}
\end{figure*}

\subsection{Experimental setups}
We conduct experiments on existing mainstream MLLMs, including both proprietary and open-source models. The parameter sizes of the open-source models range from 3.4B to 7B, 8B to 13B, and above 13B. In Table \ref{table:model-training-dataset}, we provide a detailed overview of these evaluated models in our experiments.

We employ GPT-4 as the adjudicator for LLMs to assign evaluation scores, with a focus on semantic similarity between standard answers and MLLM model outputs. Our evaluations adhere to a protocol: for reasoning and localization recognition tasks, we set the score range per question from 0 to 5. For summarization tasks, the score range per question is from 1 to 10. In the evaluation of information extraction tasks, we set the score \( s \) as 2, with an effective factor \( \delta \) of 0.8.

\subsection{Evaluation results}

We extensively evaluate open-source MLLMs models at different parameter levels and mainstream commercial MLLMs models. All detailed evaluation results are presented in Table \ref{tab:performance}. Despite significant advancements in MLLMs in recent years, they still struggle to demonstrate understanding of flowcharts, including GPT-4o. Across five different task dimensions, only the summarization task achieves relatively high scores, peaking at 82.40 points in closed-source models. However, this is only demonstrated in closed-source models; in open-source models, the highest score reaches only 74.30 points. The highest score attained in the information extraction task is only 35.30 points, while in the reasoning task, it reaches a maximum of 59.40 points. In the localization recognition task, the highest score is 48.20 points. Even under random guessing with a score of 50.00 points in the logic validation task, the highest score reaches only 83.81 points. Among all closed-source models, GPT4o demonstrates superior overall capabilities compared to other models, but only excels in the logic validation task. Among all open-source models, Phi-3-Vision achieves the highest scores, surpassing closed-source models in the information extraction task. We will further elaborate on detailed assessments across different task dimensions. Additional cases can be found in the Appendix \ref{appendix:additional example}.
\\
\textbf{Results of Information Extraction} \quad 
In this task, models generally obtain very low scores. The highest score of 35.30 is achieved by Phi-3-Vision, with the second-place model being the proprietary model Qwen-VL-MAX, but only scoring 20.32, indicating a significant gap. In Figure \ref{model prediction example}(a), for instance, by highlighting the inherent feature "pink ellipse" in the flowchart, MLLMs are enabled to extract corresponding information, with only Phi-3-Vision producing the correct answer. In Appendix \ref{appendix:Informaton-Extraction-task}, to demonstrate the performance variation of different models in Information Extraction tasks, we conduct visual analysis based on effective factors. For example, Phi-3-vision achieves an average effective factor score exceeding 0.6.
\\
\textbf{Results of Localization Recognition} \quad The evaluation results of various models in this task indicate poor performance overall, with the top performer Qwen-VL-MAX scoring only 48.20 points. In Figure \ref{model prediction example}(b), detailed examples of Qwen-VL-MAX and Phi-3-Vision are presented. The response of Qwen-VL-MAX correctly identifies the upper and lower nodes of the \textit{"Offers patient treatments and explain risks"} node as \textit{"Notify patient that cancer is diagnosed"} and \textit{"Patient choose treatment"} respectively. This indicates a clear understanding of the flowchart and the ability to accurately identify the relationships between different nodes. On the other hand, Phi-3-Vision incorrectly identifies the upper node as \textit{"Patient record"} and the lower node as \textit{"Treatment preparation."} This suggests that Phi-3-Vision struggled with accurately interpreting the connections between the nodes in the flowchart, leading to an incorrect answer.
\\
\textbf{Results of Logical Verification} \quad 
For this tasks, the open-source models LLAVA-V1.6-13B, Phi-3-Vision, LLAVA-Next-Yi-34b, and Yi-VL-34B have achieved the top two performances. Regarding the highest scoring model, GPT4o, as depicted in Figure \ref{model prediction example}(c), it exhibits concise and clear responses to questions with stronger instruction-following capabilities. Conversely, models such as CogVLM-Chat tend to generate more hallucinatory descriptions in their answers, leading to erroneous judgments. For instance, in the case of Qwen-Chat-VL, it outputs answers of the \textit{"Unknown"} type, indicating a deficiency in instruction-following capability. In Figure \ref{bar} of Appendix \ref{appendix:predicted_vs_actual}, we also analyze the predictive distributions of different models and visually compare them with the distribution of true labels. We find that the predictions of most models exhibit significant biases in this task. For example, ShareGPT4V-7B categorizes all results as correct. Only GPT4v, GPT4o, LLava-Next-Vicuna-13B, and Yi-VL-34B have prediction distributions that deviate from the actual results by no more than 15\%. Additionally, these four models consistently rank in the top five in terms of performance.
\\
\textbf{Results of Summarization} \quad
In proprietary models, the scores for this task are generally higher, with GPT4V achieving the highest score of 82.40. However, among open-source models, many still have relatively low scores. For example, MiniCPM-Llama3-V-2.5 only score 17.20, with only Phi-3-Vision, Cogvlm2-Llama3-Chat-19B, and LLAVA-Next-Yi-34B scoring above 60.00. In Figure \ref{model prediction example}(d), detailed example of LLAVA-1.5V-7B is presented. LLAVA-1.5v-7B, although detailed, provides an inaccurate and less focused response, meriting a score of 2. 
\\
\textbf{Results of Reasoning} \quad 
GPT4V achieve the best score of 59.40, yet still below a satisfactory level. In Figure \ref{model prediction example}(e), we present examples of responses from GPT4V, LLAVA-V1.6-7B, LLAVA-V1.6-13B, and Cogvlm2-Llama3-Chat-19B regarding reasoning tasks. Cogvlm2-Llama3-Chat-19B provided a more detailed response by repeating the conditions from the question and then indicating the correct next step, which may aid in accurate reasoning. LLAVA-V1.6-7B and LLAVA-V1.6-13B both provide incorrect answers to this question.


==> sec/5_futh.tex <==
\section{Further analysis}\label{sec:furthe-analysis}
In this section, we explore the impact of various factors on the FlowCE benchmark.
\subsection{Model parameter volume}
Among all open-source models, having a larger number of parameters does not necessarily lead to better performance. For instance, the 34B parameter models Yi-VL-34B and LLAVA-Next-Yi-34B scored only 26.24 and 44.33, respectively, while Phi-3-Vision, with only 4.2B parameters, achieved the best score among the open-source models. In Table \ref{table:model_A_scores}, we compare the average performance across three parameter scales. Although there may be a trend of improvement with increasing model parameters, this is not a definitive conclusion.
\subsection{Model data volume}
In Table \ref{table:model-training-dataset}, we provide detailed information on the specific pre-training and fine-tuning data volumes for each model, and further analyze how the data sources impact the performance of model on FlowCE. Despite ShareGPT4V-13B utilizing a larger dataset, its performance still lags behind LLAVA-v1.5-13B, demonstrating that the quality of the dataset is paramount. Additionally, the selection and diversity of specific datasets play a crucial role. For instance, Phi-3-Vision leverages a 0.5T image-text paired dataset that includes FLD-5B, OCR-generated synthetic data, chart comprehension datasets, and plain text data \cite{xiao2024florence, laurenccon2024obelics}. These high-quality and diverse data sources have enabled Phi-3-Vision to achieve the highest score of 35.3 in the information extraction task on FlowCE, and furthermore, it ranks first in the overall score among open-source models. 


% \subsection{Model Alignment Module}


\begin{table}[h!]
\centering
\small
\renewcommand{\arraystretch}{1}
\begin{tabular}{cc}
\toprule
\textbf{Model Parameter} & \textbf{Score} \\
\midrule
3.4B$\sim$7B & 32.47 \\
8B$\sim$13B & 31.40 \\
13B$\sim$& \textbf{35.21} \\
\bottomrule
\end{tabular}
\caption{Average Scores on FlowCE for Different Parameter Levels}
\label{table:model_A_scores}
\vspace{-5mm}
\end{table}



\subsection{Consensus between Humans and Evaluators}
In this section, we employ manual scoring evaluations for MLLMs' responses in Reasoning, Localization Recognition, and Summarization. The aim is to investigate whether the standards set by FlowCE and the use of GPT4 as an evaluator align closely with human assessment results. We engage five human evaluators to assess the model GPT4o, which emerges as the top-performing model overall. Additionally, we select the open-source model LLAVA-V1.6-13B for manual evaluation. The criteria and detailed results of the manual assessment can be found in the Appendix \ref{appendix:Manual Evaluation Protocol}. We calculate the Cohen's Kappa coefficient between the model and human evaluators, treating each score as a classification problem. The Cohen's Kappa coefficient and correlation between humans and GPT-4 when evaluating GPT-4o can reach an average of 0.90. The results indicate a significant level of agreement, demonstrating the effectiveness of our approach.



==> sec/6_con.tex <==
\section{Conclusion}
To evaluate the comprehension ability of MLLMs on flowcharts, we propose the first multi-dimensional evaluation method: FlowCE. FlowCE sets up five major categories of tasks, including reasoning, information extraction, localization recognition, logical verification, and summarization, aiming to thoroughly quantify the understanding capability and performance of MLLMs on flowcharts. The FlowCE framework not only provides an effective means to evaluate the comprehension ability of MLLMs on flowcharts, but also offers guidance for model optimization and improvement, thereby promoting the development of MLLMs.


==> sec/sup.tex <==
\clearpage
\appendix

\section{Image collection and manual annotation} \label{sec:appendix}
To obtain flowchart images, we first conducted image searches using the keyword "flowchart" on search engine(Baidu Search), and then saved them. However, we encountered issues such as duplicates, low resolution, incomplete images, and other unrelated photos. Therefore, we proceeded to manually select images, resulting in the creation of a real-world dataset.

To ensure the construction of question-answer pairs in open scenarios, we use manual annotation for each flowchart. Additionally, to ensure the diversity of the question-answer pairs, we employ a powerful GPT-like model to assist with the generation. The annotation process is illustrated in Figure \ref{fig:ap1}. Humans can choose to use GPT to generate basic diverse question-answer pairs, which are then modified as needed.

\begin{figure}[t]
%\hspace*{-6.0mm}
\centering
\includegraphics[width=2.5in]{latex/img/h-a.pdf}
    \caption{Manual annotation process, with optional assistance from GPT-like models for diversity construction.}
\label{fig:ap1}
\end{figure}
\section{Diverse Analyses of Dataset}\label{appendix:diverse analyses of dataset}
% As shown in Table \ref{tab:resolution}, the most common HD and Full HD images in daily life account for the majority of FlowCE, while other types of resolution images also have a share, indicating the diversity of FlowCE resolutions.

% \begin{table}[h]
%     \centering
%     \begin{tabular}{cc}
%         \toprule
%         \textbf{Resolution Category} & \textbf{Percentage (\%)} \\
%         \midrule
%         HD ($\leq$1280x720) & 36.8 \\
%         Full HD ($\leq$1920x1080) & 24.4 \\
%         VGA or lower ($\leq$640x480) & 16.6 \\
%         4K ($\leq$3840x2160) & 7.8 \\
%         Above 4K & 7.2 \\
%         2K ($\leq$2560x1440) & 7.2 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Resolution Categories and their Percentages}
%     \label{tab:resolution}
% \end{table}

Table \ref{tab:word_frequency} is a preview of the first five rows of the word frequency statistics table. The following conclusions can be drawn from the analysis of the word frequency statistics table:
\begin{itemize}
    \item \textbf{High number of unique words:} The data contains 8046 different words, indicating that the flowchart involves a large number of different operations and entities.
    
    \item \textbf{Broad frequency distribution:} The total word frequency is 23994 times, with each word appearing an average of about 2.98 times. This shows the wide usage of vocabulary, with no single word dominating the entire flowchart.
    
    \item \textbf{Specific word types and frequency analysis:} 
    \begin{itemize}
        \item Includes various operations such as "start," "receive," and "send." These verbs indicate that the flowchart covers various steps and activities from start to finish.
        \item Includes various entities such as "data," "customer," and "decision." These nouns show that the flowchart involves data processing, customer interactions, decision points, task management, and approval processes.
    \end{itemize}
    
    \item \textbf{Extremes in word usage frequency:} 
    \begin{itemize}
        \item Highest frequency word: "no" appears 631 times, indicating a large number of negative judgments or conditions in the flowchart.
        \item Lowest frequency words: There are 4703 words that appear only once, indicating the presence of many unique and rare operations and entities in the flowchart.
    \end{itemize}
\end{itemize}

\begin{table}[h]
    \centering
    \begin{tabular}{ccccccc}
        \toprule
        \textbf{Word} & no & yes & the & to & and & $\cdots$ \\
        \midrule
        \textbf{Frequency} & 631 & 622 & 510 & 384 & 271 & $\cdots$ \\
        \bottomrule
    \end{tabular}
    \caption{Top 5 Word Frequencies in Flowcharts}
    \label{tab:word_frequency}
\end{table}

We randomly selected 100 flowcharts for statistical analysis. Table \ref{tab:arg_nodes_edges} show that each flowchart contains an average of 10.56 node boxes and 11.64 logical edges. This indicates that our flowcharts are sufficiently complex on average. Additionally, the flowchart with the most node boxes contains 38 node boxes and 36 logical edges.

The distribution of node boxes and logical edges is as follows:

\begin{enumerate}[label=\alph*)]
    \item \textbf{Distribution of node boxes:} The number of node boxes in most flowcharts ranges from 5 to 15, with a few flowcharts having more than 20 node boxes, reaching a maximum of 38.
    
    \item \textbf{Distribution of logical edges:} The number of logical edges is mainly between 5 and 15, with a few flowcharts having more than 20 logical edges, reaching a maximum of 36.
\end{enumerate}



\begin{table}[h]
    \centering
    \begin{tabular}{cc}
        \toprule
        \textbf{Arg. Nodes} & \textbf{Arg. Edges} \\
        \midrule
        10.56 & 11.64 \\
        \bottomrule
    \end{tabular}
    \caption{Average Number of Nodes and Edges in Flowcharts}
    \label{tab:arg_nodes_edges}
\end{table}


\section{Large Language Model Judge} \label{appendix:Large Language Model Judge}
We use GPT-4 as an automated evaluator to score tasks in three categories: localization recognition, reasoning, and summarization. The scoring methodology is illustrated in Figure \ref{eval}, where we set a score range of 0-5 for each question in the reasoning and localization recognition tasks, and a score range of 1-10 for the summarization tasks.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.00\textwidth]{latex/img/eval.pdf} 
    \caption{
Using GPT-4 as an automated evaluator.
}
    \label{eval}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.70\textwidth]{latex/img/case1.pdf} 
    \caption{
Model output and received scores.
}
    \label{1c}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.70\textwidth]{latex/img/case2.pdf} 
    \caption{
Model output and received scores.
}
    \label{2c}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.70\textwidth]{latex/img/case3.pdf} 
    \caption{
Model output and received scores.
}
    \label{3c}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.70\textwidth]{latex/img/more-example-ie.pdf} 
    \caption{
Model output and received scores.
}
    \label{4c}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.70\textwidth]{latex/img/more-example-veri.pdf} 
    \caption{
Model output and received scores.
}
    \label{5c}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.70\textwidth]{latex/img/more-example-summary.pdf} 
    \caption{
Model output and received scores.
}
    \label{6c}
\end{figure*}



\section{Additional examples} \label{appendix:additional example}
We provide more examples in Figures \ref{1c}, \ref{2c}, \ref{3c}, \ref{4c}, \ref{5c} and \ref{6c}, including the model's responses and the evaluation scores given by GPT-4. 

\section{Manual Evaluation Protocol} \label{appendix:Manual Evaluation Protocol}
We provide both the standard answers from FlowCE and the model's output answers. In Table \ref{tab:human-gpt}, we present the scoring results for GPT-4o and LLAVA by humans and GPT-4 in the RS, LR, and SM tasks (note that the subjective scoring tasks are only RS, LR, and SM). We then calculate the Pearson correlation coefficient for each row in the table based on these overall score results. In Table \ref{table:model_A_scores}, we present the Pearson correlation coefficients between human ratings and GPT4 scores under our answer setting. The results demonstrate a high degree of consistency between human evaluation and our assessment methodology, indicating that our FlowCE evaluation results can be regarded as effective assessments. In Table \ref{tab:cohens_kappa}, we include Cohen's Kappa between the LLM and humans, treating each score as a classification problem. The Cohen's Kappa between humans and GPT-4 for evaluating GPT-4o is 0.54, and for evaluating LLAVA is 0.49. The results show a certain level of agreement, but given our wide score range and the high subjectivity of open-ended Q\&A, we consider this level of agreement to be valid. 




\textbf{RS and LR Tasks:}
\\
5 points: Answer is entirely correct with no factual errors.
\\
4 points: Answer is mostly correct with minor factual errors that do not affect the main content.
\\
3 points: Answer contains some factual errors but is still useful overall.
\\
2 points: Answer has significant factual errors, with some content being incorrect.
\\
1 point: Answer is severely flawed, with most content being incorrect.
\\
0 points: Completely incorrect.
\\
\textbf{SM Task:} 
\\
10 points: The answer is completely correct without any factual errors.
\\
8 points: The answer is basically correct with only minor factual errors that do not affect the main content.
\\
6 points: The answer contains some factual errors but is still useful on the whole.
\\
4 points: The answer has significant factual errors with incorrect parts of the content.
\\
2 points: The answer is seriously incorrect with most of the content incorrect.
\\
1 point: The answer is completely incorrect.

\begin{table}[h!]
    \footnotesize
    \centering
    \begin{tabular}{cccccccc}
        \toprule
        Model & \multicolumn{3}{c}{GPT4-score} & \multicolumn{3}{c}{Human-score} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
         & RS & LR & SM & RS & LR & SM \\
        \midrule
        GPT4o & 57.6 & 44.8 & 79.9 & 62.6 & 58.4 & 75.9 \\
        LLAVA & 37.4 & 27.8 & 50.7 & 45.8 & 36.8 & 47.6 \\
        \bottomrule
    \end{tabular}
    \caption{Performance Comparison between GPT4o and LLAVA.}
    \label{tab:human-gpt}
\end{table}


% \begin{table}[h]
%     \centering
%     \begin{tabular}{ccc}
%         \hline
%         \textbf{Cohen's Kappa} & \textbf{GPT-4o} & \textbf{LLAVA} \\
%         \hline
%         Human and GPT-4 & 0.54 & 0.49 \\
%         \hline
%     \end{tabular}
%     \caption{Cohen's Kappa Agreement Scores between Human Evaluators and LLMs (GPT-4o and LLAVA)}
%     \label{tab:cohens_kappa}
% \end{table}

\begin{table}[h!]
    \centering
    \small
    \begin{tabular}{cccc}
    \toprule
     & \textbf{RS} & \textbf{LR} & \textbf{SM}\\
    \midrule
    \textbf{Correlation} & 0.97 & 0.97 & 0.91 \\
    \bottomrule
    \end{tabular}
    \caption{The Pearson correlation coefficient between human ratings and GPT4 scores for various tasks.}
    \label{table:model_A_scores}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{ccc}
        \hline
        \textbf{Cohen's Kappa} & \textbf{GPT-4o} & \textbf{LLAVA} \\
        \hline
        Human and GPT-4 & 0.54 & 0.49 \\
        \hline
    \end{tabular}
    \caption{Cohen's Kappa Agreement Scores between Human Evaluators and LLMs (GPT-4o and LLAVA)}
    \label{tab:cohens_kappa}
\end{table}

\section{Detailed Comparison of Logical Verification Task} \label{appendix:predicted_vs_actual}
In this section, we present a detailed comparison of the predicted results for a subset of models: GPT4o, Phi-3-Vision, LLaVA-Next-Vicuna-13B, Qwen-Chat-VL, LLaVA-Next-Vicuna-7B, LLaVA-V1.5-13B, Cogvlm2-Llama3-Chat-19B, and Cogvlm-Chat. 
\begin{figure*}[h]
    \centering
    \includegraphics[width=1.00\textwidth]{latex/img/bar.pdf} 
    \caption{
The prediction distributions of different models on the logical verification task.
}
    \label{bar}
\end{figure*}
Each subplot in Figure \ref{bar} compares the predicted results (in blue) with the actual answer labels (in red) for each model. The score below each subplot indicates the overall performance of the model based on its accuracy in predicting the correct category.

GPT4o stands out with the highest accuracy, achieving a score of 83.81, indicating robust performance in aligning predictions with actual labels. Phi-3-Vision, while scoring 60.95, demonstrates a noticeable discrepancy in the \textit{"No"} category with lower prediction accuracy. LLaVA-Next-Vicuna-13B, with a score of 62.86, shows moderate alignment but also exhibits substantial errors in the \textit{"No"} category. Qwen-Chat-VL and Cogvlm-Chat, both scoring 50.48, indicate significant prediction errors and lower overall accuracy, particularly evident in the \textit{"No"} and \textit{"Unknown"} categories. LLaVA-Next-Vicuna-7B and LLaVA-V1.5-13B, scoring 52.38 and 53.55 respectively, also reflect moderate performance but with specific inaccuracies in the \textit{"No"} category. Cogvlm2-Llama3-Chat-19B, with a score of 57.14, shows better performance than some other models but still falls short in accurately predicting the \textit{"No"} responses. These results suggest that while certain models like GPT4o exhibit strong performance, others require significant improvements in understanding and predicting both \textit{"Yes"} and \textit{"No"} categories accurately. The varying scores underscore the necessity for further refinement in training methodologies and model architectures to enhance predictive accuracy across all categories.

The phenomenon where some models exhibit a near 100\% probability in answering \textit{"Yes"} can be attributed to several factors:

\begin{figure*}[h]
    \centering
    \includegraphics[width=1.00\textwidth]{latex/img/scatter.pdf} 
    \caption{
Comparison of MLLMs Performance on Information Extraction tasks based on effective factor distribution. The red line represents the smoothed ascending order of the average effective factor across all models for each specific question. The orange line indicates the average effective factor for each model across all question.
}
    \label{scatter}
\end{figure*}


\begin{itemize}
    \item \textbf{Training Data Bias}: The training datasets may have an imbalance where affirmative answers (\textit{"Yes"}) are disproportionately represented compared to negative ones (\textit{"No"}). This bias in the training data can lead the models to favor \textit{"Yes"} responses, as they learn to associate the affirmative answer with higher probabilities during the training process.
    
    \item \textbf{Model Overfitting}: Certain models might be overfitted to specific patterns in the training data, especially if those patterns predominantly involve affirmative responses. Overfitting can cause the model to generalize poorly to new, unseen data, resulting in a high likelihood of predicting \textit{"Yes"} regardless of the actual context or question.
    
    \item \textbf{Algorithmic Tuning}: The hyperparameters and algorithmic settings of some models might be tuned in a way that inadvertently biases the model towards affirmative responses. This could include settings related to decision thresholds, loss functions, or other optimization parameters that skew the model's predictions towards \textit{"Yes"}.
    
    \item \textbf{Lack of Contextual Understanding}: Some models may lack the nuanced understanding required to accurately discern between \textit{"Yes"} and \textit{"No"} in complex scenarios. This deficiency can lead them to default to a \textit{"Yes}" answer, especially if they are not effectively capturing and processing the context of the queries.
    
    \item \textbf{Evaluation Metrics}: The evaluation metrics used during the training and validation phases might inadvertently prioritize accuracy in affirmative answers due to the distribution of the training data. This focus on affirmative accuracy can lead the models to perform better on \textit{"Yes"} predictions, inflating the probability of such responses in practical applications.
\end{itemize}

These factors collectively contribute to the observed high probability of \textit{"Yes"} responses in some models, highlighting the need for balanced training data, careful tuning, and improved contextual understanding in model development.




\section{Detailed Comparison of Informaton Extraction Task} \label{appendix:Informaton-Extraction-task}

As shown in Figure \ref{scatter}, there are notable differences in the distribution of effective factor values among various models. Phi-3-Vision and GPT-4 have a broad distribution of effective factor values, with more data points in the higher effective factor region (above 0.6). Other models have a more scattered distribution of effective factor values, with most concentrated in the low effective factor region, particularly Qwen-Chat-VL, where the majority of data points are below 0.2. Despite the Cogvlm family having relatively high effective factors and fewer incorrect answers, the overall number of labels is also small. After subtracting the incorrect labels, the number of correct labels is minimal, resulting in a very low total score.


\section{Limitations}
This work has two limitations. Firstly, it establishes the FlowCE benchmark based on flowcharts derived from a diverse set of 500 real-world images. While it poses challenges for existing closed-source and open-source models, continuous expansion of both the dataset size and the number of questions is necessary going forward. Secondly, FlowCE relies entirely on manual annotation for data generation. However, as the dataset grows, dependence on manual annotation introduces inherent limitations, making it difficult to completely eliminate errors from the data.
